Multifaceted Hierarchical Report Identification for Non-Functional Bugs in Deep Learning Frameworks

Non-functional bugs (e.g., performance- or accuracy-related bugs) in Deep Learning (DL) frameworks can lead to some of the most devastating consequences. Reporting those bugs on a repository such as GitHub is a standard route to fix them. Yet, given the growing number of new GitHub reports for DL frameworks, it is intrinsically difficult for developers to distinguish those that reveal non-functional bugs among the others, and assign them to the right contributor for investigation in a timely manner. In this paper, we propose MHNurf - an end-to-end tool for automatically identifying non-functional bug related reports in DL frameworks. The core of MHNurf is a Multifaceted Hierarchical Attention Network (MHAN) that tackles three unaddressed challenges: (1) learning the semantic knowledge, but doing so by (2) considering the hierarchy (e.g., words/tokens in sentences/statements) and focusing on the important parts (i.e., words, tokens, sentences, and statements) of a GitHub report, while (3) independently extracting information from different types of features, i.e., content, comment, code, command, and label. To evaluate MHNurf, we leverage 3,721 GitHub reports from five DL frameworks for conducting experiments. The results show that MHNurf works the best with a combination of content, comment, and code, which considerably outperforms the classic HAN where only the content is used. MHNurf also produces significantly more accurate results than nine other state-of-the-art classifiers with strong statistical significance, i.e., up to 71% AUC improvement and has the best Scott-Knott rank on four frameworks while 2nd on the remaining one. To facilitate reproduction and promote future research, we have made our dataset, code, and detailed supplementary results publicly available at: https://github.com/ideas-labo/APSEC2022-MHNurf.

==> fig/exp3-copy.tex <==
% CS Table for RQ2
\begin{table*}[!b]
    \caption{Scott-Knott analysis results of experiment 3 for five open-source deep learning system projects.}
    \label{tbl:opensourceResultCS}
  \begin{center}
    \begin{adjustbox}{max width = \textwidth}
     

    \begin{tabular}{c@{}c@{}c}
        \begin{tabular}{lcccl}
            \cellcolor[gray]{1}\textbf{algorithm} & \cellcolor[gray]{1}\textbf{rank} &     \cellcolor[gray]{1}\textbf{med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
            HAN(title+desc)+comment+code & 1 & 0.857 & 0.025 &  \quart{84.5}{2.5}{85.7}{100}\\
            HAN(title+desc) & 1 & 0.854 & 0.036 & \quart{83.7}{3.6}{85.4}{100} \\
            TF-IDF + MLP & 2 & 0.790 & 0.023 & \quart{78.1}{2.3}{79}{100} \\
            fastText + autotune & 3 & 0.786 & 0.039 & \quart{76.1}{3.9}{78.6}{100} \\
            TF-IDF + NB & 4 & 0.771 & 0.035 & \quart{74.8}{3.5}{77.1}{100} \\
            CNN & 5 & 0.700 & 0.070 & \quart{65.6}{7}{70}{100} \\
            LSTM & 6 & 0.681 & 0.102 & \quart{60.7}{10.2}{68.1}{100} \\
            TF-IDF + RF & 7 & 0.653 & 0.043 & \quart{62.7}{4.3}{65.3}{100} \\
            TF-IDF + KNN & 7 & 0.619 & 0.053 & \quart{59.6}{5.3}{61.9}{100} \\
            TF-IDF + SVM & 8 & 0.500 & 0.148 & \quart{50}{14.8}{50}{100} \\
            fastText & 9 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
        \end{tabular} & 
        \begin{tabular}{|lcccl}
           \cellcolor[gray]{1}\textbf{algorithm} & \cellcolor[gray]{1}\textbf{rank} &     \cellcolor[gray]{1}\textbf{med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
            HAN(title+desc) & 1 & 0.757 & 0.034 & \quart{73.6}{3.4}{75.7}{100} \\
            HAN(title+desc)+comment+code & 2 & 0.748 & 0.046 & \quart{72.6}{4.6}{74.8}{100}  \\
            TF-IDF + NB & 3 & 0.725 & 0.041 & \quart{70.7}{4.1}{72.5}{100} \\
            TF-IDF + MLP & 4 & 0.640 & 0.108 & \quart{58.8}{10.8}{64}{100} \\
            fastText + autotune & 5 & 0.557 & 0.108 & \quart{50.4}{10.8}{55.7}{100} \\
            TF-IDF + SVM & 5 & 0.500 & 0.150 & \quart{50}{15}{50}{100} \\
            TF-IDF + RF & 6 & 0.539 & 0.035 & \quart{52}{3.5}{53.9}{100} \\
            CNN & 6 & 0.518 & 0.077 & \quart{50}{7.7}{51.8}{100} \\
            TF-IDF + KNN & 7 & 0.500 & 0.027 & \quart{50}{2.7}{50}{100} \\
            LSTM & 8 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
            fastText & 9 & 0.500 & 0.000 &  \\
        \end{tabular} &
        \begin{tabular}{|lcccl}
            \cellcolor[gray]{1}\textbf{algorithm} & \cellcolor[gray]{1}\textbf{rank} &     \cellcolor[gray]{1}\textbf{med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1} \\
            \hline
             HAN(title+desc)+comment+code & 1 & 0.828 & 0.093 & \quart{77.4}{9.3}{82.8}{100} \\
            HAN(title+desc) & 2 & 0.815 & 0.067 & \quart{77.8}{6.7}{81.5}{100} \\
            TF-IDF + NB & 3 & 0.781 & 0.054 & \quart{74.9}{5.4}{78.1}{100} \\
            TF-IDF + MLP & 4 & 0.714 & 0.069 & \quart{69}{6.9}{71.4}{100} \\
            fastText + autotune & 5 & 0.708 & 0.058 & \quart{69}{5.8}{70.8}{100} \\
            TF-IDF + RF & 6 & 0.643 & 0.066 & \quart{60.4}{6.6}{64.3}{100} \\
            TF-IDF + SVM & 7 & 0.611 & 0.090 & \quart{57.7}{9}{61.1}{100} \\
            CNN & 8 & 0.617 & 0.057 & \quart{58.2}{5.7}{61.7}{100} \\
            LSTM & 8 & 0.592 & 0.121 & \quart{53.5}{12.1}{59.2}{100} \\
            TF-IDF + KNN & 9 & 0.582 & 0.058 & \quart{56.7}{5.8}{58.2}{100} \\
            fastText & 10 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
        \end{tabular} \\
        \textbf{(a). TensorFlow} & \textbf{(b). PyTorch} & \textbf{(c). Keras}
        \\
        \\
        \begin{tabular}{lcccl}
             \cellcolor[gray]{1}\textbf{algorithm} & \cellcolor[gray]{1}\textbf{rank} &     \cellcolor[gray]{1}\textbf{med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}
            \\
            \hline
            HAN(title+desc)+comment+code & 1 & 0.778 & 0.199 & \quart{67.3}{19.9}{77.8}{100} \\
            TF-IDF + NB & 1 & 0.770 & 0.051 & \quart{73.6}{5.1}{77}{100} \\
            HAN(title+desc) & 2 & 0.744 & 0.350 & \quart{50}{35}{74.4}{100} \\
            TF-IDF + MLP & 3 & 0.659 & 0.078 & \quart{61}{7.8}{65.9}{100} \\
            fastText + autotune & 4 & 0.616 & 0.085 & \quart{58.8}{8.5}{61.6}{100} \\
            TF-IDF + KNN & 5 & 0.538 & 0.070 & \quart{50.6}{7}{53.8}{100} \\
            TF-IDF + SVM & 5 & 0.500 & 0.099 & \quart{50}{9.9}{50}{100} \\
            TF-IDF + RF & 6 & 0.500 & 0.034 & \quart{50}{3.4}{50}{100} \\
            CNN & 6 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
            LSTM & 6 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
            fastText & 7 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
        \end{tabular} &

        \begin{tabular}{|lcccl|}
            \cellcolor[gray]{1}\textbf{algorithm} & \cellcolor[gray]{1}\textbf{rank} &     \cellcolor[gray]{1}\textbf{med} & \cellcolor[gray]{1}\textbf{IQR} & \cellcolor[gray]{1}\\
            \hline
            TF-IDF + NB & 1 & 0.665 & 0.060 & \quart{64.7}{6}{66.5}{100} \\
            HAN(title+desc)+comment+code & 2 & 0.646 & 0.247 & \quart{50}{24.7}{64.6}{100} \\
            HAN(title+desc) & 2 & 0.652 & 0.228 & \quart{50}{22.8}{65.2}{100} \\
            TF-IDF + MLP & 3 & 0.590 & 0.102 & \quart{56.5}{10.2}{59}{100} \\
            fastText + autotune & 4 & 0.586 & 0.068 & \quart{56.7}{6.8}{58.6}{100} \\
            TF-IDF + KNN & 5 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
            TF-IDF + SVM & 5 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
            LSTM & 6 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
            fastText & 7 & 0.500 & 0.000 &  \quart{50}{0}{50}{100}\\
            TF-IDF + RF & 8 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
            CNN & 9 & 0.500 & 0.000 & \quart{50}{0}{50}{100} \\
        \end{tabular} &
        \begin{tabular}{lc}
            \cellcolor[gray]{1}\textbf{algorithm} & \cellcolor[gray]{1}\textbf{rank}\\
            \hline
            HAN(title+desc)+comment+code& \hphantom{you can't see me!!}7\hphantom{you can't see me!!} \\
            HAN(title+desc) & 8 \\
            TF-IDF + NB & 12 \\
            TF-IDF + MLP & 16 \\
            fastText + autotune & 21 \\
            TF-IDF + SVM & 30 \\
            TF-IDF + KNN & 33 \\
            TF-IDF + RF & 33 \\
            CNN & 34 \\
            LSTM & 34 \\
            fastText & 42 \\
        \end{tabular}\\
        \textbf{(d). MXNet}  & \textbf{(e). Caffe} & \textbf{(f). RankSum}\\
    \end{tabular}
  \end{adjustbox}
   \end{center}
\end{table*}

==> tab/approaches.tex <==
% \begin{table}[t!]
% \centering
%   \caption{The existing approaches used in the experiment.}
%   \label{tab:approaches}
%   \footnotesize
%   \begin{tabular}
%     \toprule
%     \textbf{Method (Reference)}&\textbf{Interpretation}\\
%     \midrule
%     TF-IDF + $k$NN (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& $k$-Nearest Neighbors  is an simple algorithm that assigns the inputs to the class that is the most common among its $k$ nearest neighbors. \\
%     \midrule
%     TF-IDF + MLP (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21}) & MultiLayer Perceptrons (MLP) is a supplement of feed forward neural network which consists of input layer, output layer and hidden layer. \cite{DBLP:journals/ac/AbiramiC20}. \\
%     \midrule
%     TF-IDF + NB
%     (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& Naïve Bayes (NB) replies on the Bayes Theorem to classify the instances with assumptions on the interdependence between data attributes.  \\
%     \midrule
%     TF-IDF + RF (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& Random Forest (RF) is an ensemble learning algorithm which is constructed by multiple decision tree \cite{DBLP:conf/cores/ZolnierekR05}. \\
%     \midrule
%     TF-IDF + SVM (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& Support Vector Machine (SVM) relies on a chosen nonlinear kernel function to transform the datainto a high dimension feature space, within which the data may become separable for classification \cite{wang2005support}.\\
%     \midrule
%     TextCNN (\citeauthor{DBLP:journals/tr/UmerLI20}~\cite{DBLP:journals/tr/UmerLI20}) & \\
%     \midrule
%     LSTM (\citeauthor{DBLP:conf/icmla/0003FWBL18}~\cite{DBLP:conf/icmla/0003FWBL18}) & \\
%     \midrule
%     fastText (\citeauthor{DBLP:conf/icsm/KallisSCP19}~\cite{DBLP:conf/icsm/KallisSCP19}) & \\
%     \midrule
%     fastText + autoTune (\citeauthor{DBLP:journals/ese/HerboldTT20}~\cite{DBLP:journals/ese/HerboldTT20}) & \\
%   \bottomrule
%  \end{tabular}
% % \begin{tablenotes}
% %     In the table, TF-IDF represents Term Frequency - Inverse Document Frequency. $k$NN represents $k$-nearest neighbors. MLP represents MultiLayer Perceptron. NB represents Naïve Bayes. RF represents Random Forest. SVM represents Support Vector Machine. CNN represents Convolutional Neural Networks. LSTM represents Long Short-Term Memory.
% % \end{tablenotes}
% \end{table}

\begin{table*}
  \caption{The existing approaches used in the experiment.}
  \label{tab:freq}
  \footnotesize
\begin{threeparttable}
  \begin{tabular}{l p{13cm}}
    \toprule
    \textbf{Method (Reference)}&\textbf{Interpretation}\\
    \midrule
    
    TF-IDF + $k$NN (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& $k$-Nearest Neighbors ($k$NN) is a simple algorithm that assigns the inputs to the class that is the $k$ most common. \\

    TF-IDF + MLP (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21}) & MultiLayer Perceptrons (MLP) is a supplement of feed forward neural network which consists of input, output and hidden layer. \cite{DBLP:journals/ac/AbiramiC20}. \\

    TF-IDF + NB
    (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& Naïve Bayes (NB) replies on Bayes Theorem to classify instances with assumptions on the interdependence between data attributes.  \\

    TF-IDF + RF (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& Random Forest (RF) is an ensemble learning algorithm which is constructed by multiple decision tree \cite{DBLP:conf/cores/ZolnierekR05}. \\

    TF-IDF + SVM (\citeauthor{DBLP:journals/infsof/GomesTC21}~\cite{DBLP:journals/infsof/GomesTC21})& Support Vector Machine (SVM) is an algorithm using nonlinear kernel to transform data into a high dimension feature space.\\

    TextCNN (\citeauthor{DBLP:journals/tr/UmerLI20}~\cite{DBLP:journals/tr/UmerLI20}) & TextCNN is a convolutional neural network for text, which is a useful deep learning algorithm for sentence classification tasks \cite{DBLP:conf/emnlp/Kim14}.\\

    LSTM (\citeauthor{DBLP:conf/icmla/0003FWBL18}~\cite{DBLP:conf/icmla/0003FWBL18}) & Long short-term memory (LSTM) networks are recurrent neural networks that can remember patterns for long duration of time \cite{roshan2020violence}. \\

    fastText (\citeauthor{DBLP:conf/icsm/KallisSCP19}~\cite{DBLP:conf/icsm/KallisSCP19}) & fastText is a lightweight library that allows to use efficient text classification with bag of tricks \cite{DBLP:conf/eacl/GraveMJB17}.\\

    fastText + autoTune (\citeauthor{DBLP:journals/ese/HerboldTT20}~\cite{DBLP:journals/ese/HerboldTT20}) & AutoTune is fastText's Automatic hyperparameter optimization which allows user to find automatically the best hyperparameters.\\
  \bottomrule
\end{tabular}
\begin{tablenotes}
        % \singlespacing
        \footnotesize
        \item[*] TF-IDF represents term frequency–inverse document frequency. It is a numerical statistic used for reflecting the importance of a word to a document in a  corpus \cite{rajaraman2011mining}.
    \end{tablenotes}
  \end{threeparttable}
\end{table*}

==> tab/code-exp.tex <==
\begin{document}
\begin{minted}{python}
import numpy as np
    
def incmatrix(genl1,genl2):
    m = len(genl1)
    n = len(genl2)
    M = None #to become the incidence matrix
    VT = np.zeros((n*m,1), int)  #dummy variable
    
    #compute the bitwise xor matrix
    M1 = bitxormatrix(genl1)
    M2 = np.triu(bitxormatrix(genl2),1) 

   
\end{minted}
\end{document}

==> tab/exp1.tex <==
\begin{table}[h]
    \footnotesize
    \label{tab:temps}
    \caption{The result of experiment 1}
    \setlength{\tabcolsep}{1mm}
    \begin{subtable}[h]{0.25\textwidth}
        \centering
        \begin{tabular}{llllll}
        \toprule
         \rotatebox{90}{\textbf{Textual Feature}}& \rotatebox{90}{\textbf{TensorFlow}} &  \rotatebox{90}{\textbf{PyTorch}} & \rotatebox{90}{\textbf{Keras}} & \rotatebox{90}{\textbf{Mxnet
        }} & \rotatebox{90}{\textbf{Caffe}}\\
        \midrule
        title & 0.841 & 0.615 & 0.720 & 0.623 & 0.575 \\
        desc & 0.769 & 0.610 & 0.674 & 0.628 & 0.581 \\
        title+desc & 0.854 & 0.646 & 0.787 & 0.703 & 0.641 \\
        \bottomrule
        \end{tabular}
       \caption{AUC values}
       \label{tab:week1}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.2\textwidth}
        \centering
        \begin{tabular}{llllll}
        \toprule
         \rotatebox{90}{\textbf{Textual Feature}}& \rotatebox{90}{\textbf{TensorFlow}} &  \rotatebox{90}{\textbf{PyTorch}} & \rotatebox{90}{\textbf{Keras}} & \rotatebox{90}{\textbf{Mxnet
        }} & \rotatebox{90}{\textbf{Caffe}}\\
        \midrule
        title & 2 & 2 & 2 & 2 & 2 \\
        desc & 3 & 2 & 3 & 2 & 2 \\
        title+desc & 1 & 1 & 1 & 1 & 1\\
        \bottomrule
        \end{tabular}
        \caption{ScottKnottESD Rank}
        \label{tab:week2}
     \end{subtable}
\end{table}


==> tab/exp2.tex <==
\begin{table}[h]
    \footnotesize
    \label{tab:temps}
    \caption{The result of experiemnt 2 (The AUC values are filled with gradient color from dark blue to white according to their values from the highest to lowest in a  certain project).}
    \setlength{\tabcolsep}{1mm}
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{llllllllllllll}
\toprule
 \textbf{Network Combination}& \rotatebox{90}{\textbf{TensorFlow}} &  \rotatebox{90}{\textbf{PyTorch}} & \rotatebox{90}{\textbf{Keras}} & \rotatebox{90}{\textbf{Mxnet
}} & \rotatebox{90}{\textbf{Caffe}}\\
\midrule
HAN(title+desc) & \cellcolor[HTML]{3C9EE0}0.854 & \cellcolor[HTML]{F5FAFD}0.646 & \cellcolor[HTML]{C8E3F6}0.79 & \cellcolor[HTML]{F5FAFD}0.703 & \cellcolor[HTML]{56ABE4}0.641 \\
HAN(title+desc)+code & \cellcolor[HTML]{8BC5ED}0.851 & \cellcolor[HTML]{2392DD}0.679 & \cellcolor[HTML]{1D7AB9}0.818 & \cellcolor[HTML]{B6DAF2}0.731 & \cellcolor[HTML]{AAD4F0}0.629 \\
HAN(title+desc)+code+command & \cellcolor[HTML]{B6DAF2}0.848 & \cellcolor[HTML]{65B2E7}0.672 & \cellcolor[HTML]{E9F3FB}0.781 & \cellcolor[HTML]{AAD4F0}0.735 & \cellcolor[HTML]{1F84C9}0.65 \\
HAN(title+desc)+code+command+label & \cellcolor[HTML]{E9F3FB}0.844 & \cellcolor[HTML]{56ABE4}0.674 & \cellcolor[HTML]{78BCEA}0.803 & \cellcolor[HTML]{65B2E7}0.748 & \cellcolor[HTML]{99CCEF}0.636 \\
HAN(title+desc)+code+label & \cellcolor[HTML]{99CCEF}0.851 & \cellcolor[HTML]{C8E3F6}0.66 & \cellcolor[HTML]{65B2E7}0.804 & \cellcolor[HTML]{8BC5ED}0.739 & \cellcolor[HTML]{B6DAF2}0.621 \\
HAN(title+desc)+command & 0.844 & \cellcolor[HTML]{D6EAF8}0.656 & \cellcolor[HTML]{99CCEF}0.8 & \cellcolor[HTML]{99CCEF}0.735 & \cellcolor[HTML]{78BCEA}0.637 \\
HAN(title+desc)+command+label & \cellcolor[HTML]{AAD4F0}0.849 & 0.644 & 0.766 & \cellcolor[HTML]{56ABE4}0.749 & \cellcolor[HTML]{3C9EE0}0.642 \\
HAN(title+desc)+comment & \cellcolor[HTML]{2392DD}0.856 & \cellcolor[HTML]{1F84C9}0.687 & \cellcolor[HTML]{1F84C9}0.808 & 0.702 & \cellcolor[HTML]{2392DD}0.646 \\
HAN(title+desc)+comment+code & \cellcolor[HTML]{1F84C9}0.857 & \cellcolor[HTML]{3C9EE0}0.676 & \cellcolor[HTML]{56ABE4}0.804 & \cellcolor[HTML]{2392DD}0.75 & \cellcolor[HTML]{1D7AB9}0.653 \\
HAN(title+desc)+comment+code+command & \cellcolor[HTML]{56ABE4}0.853 & \cellcolor[HTML]{99CCEF}0.665 & \cellcolor[HTML]{D6EAF8}0.787 & \cellcolor[HTML]{1D7AB9}0.768 & 0.594 \\
HAN(title+desc)+comment+code+command+label & \cellcolor[HTML]{78BCEA}0.851 & \cellcolor[HTML]{AAD4F0}0.663 & \cellcolor[HTML]{3C9EE0}0.805 & \cellcolor[HTML]{C8E3F6}0.73 & \cellcolor[HTML]{F5FAFD}0.606 \\
HAN(title+desc)+comment+code+label & \cellcolor[HTML]{F5FAFD}0.844 & \cellcolor[HTML]{B6DAF2}0.661 & \cellcolor[HTML]{8BC5ED}0.803 & \cellcolor[HTML]{E9F3FB}0.719 & \cellcolor[HTML]{E9F3FB}0.607 \\
HAN(title+desc)+comment+command & \cellcolor[HTML]{D6EAF8}0.846 & \cellcolor[HTML]{8BC5ED}0.665 & \cellcolor[HTML]{AAD4F0}0.793 & \cellcolor[HTML]{1F84C9}0.764 & \cellcolor[HTML]{D6EAF8}0.618 \\
HAN(title+desc)+comment+command+label & \cellcolor[HTML]{C8E3F6}0.846 & \cellcolor[HTML]{E9F3FB}0.653 & \cellcolor[HTML]{2392DD}0.807 & \cellcolor[HTML]{3C9EE0}0.749 & \cellcolor[HTML]{C8E3F6}0.619 \\
HAN(title+desc)+comment+label & \cellcolor[HTML]{1D7AB9}0.859 & \cellcolor[HTML]{1D7AB9}0.687 & \cellcolor[HTML]{F5FAFD}0.773 & \cellcolor[HTML]{78BCEA}0.748 & \cellcolor[HTML]{8BC5ED}0.637 \\
HAN(title+desc)+label & \cellcolor[HTML]{65B2E7}0.852 & \cellcolor[HTML]{78BCEA}0.668 & \cellcolor[HTML]{B6DAF2}0.79 & \cellcolor[HTML]{D6EAF8}0.729 & \cellcolor[HTML]{65B2E7}0.64 \\
% \textbf{PERCENT} & 13.0\% & 0.2\% & 28.0\% & 0.9\% & 0.9\% & 1.4\% & 7.2\% & 4.4\% & 5.6\% & 8.4\% & 5.4\% & 24.7\%\\
\bottomrule
\end{tabular}
       \caption{AUC Values}
       \label{tab:week1}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{llllllllllllll}
        \toprule
        \textbf{Network Combination}& \rotatebox{90}{\textbf{TensorFlow}} &  \rotatebox{90}{\textbf{PyTorch}} & \rotatebox{90}{\textbf{Keras}} & \rotatebox{90}{\textbf{Mxnet
        }} & \rotatebox{90}{\textbf{Caffe}}&  \rotatebox{90}{\textbf{RankSum}}\\
        \midrule
HAN(title+desc)+comment+code & 1 & 2 & 2 & 1 & 1 & 7 \\
HAN(title+desc)+comment+label & 1 & 1 & 4 & 1 & 1 & 8 \\
HAN(title+desc)+comment & 1 & 1 & 2 & 3 & 1 & 8 \\
HAN(title+desc)+code & 2 & 2 & 1 & 2 & 1 & 8 \\
HAN(title+desc)+code+command+label & 3 & 2 & 2 & 1 & 1 & 9 \\
HAN(title+desc)+label & 2 & 2 & 3 & 2 & 1 & 10 \\
HAN(title+desc)+code+label & 2 & 3 & 2 & 1 & 2 & 10 \\
HAN(title+desc)+code+command & 3 & 2 & 3 & 2 & 1 & 11 \\
HAN(title+desc)+command & 3 & 3 & 2 & 2 & 1 & 11 \\
HAN(title+desc)+comment+code+command & 2 & 3 & 3 & 1 & 3 & 12 \\
HAN(title+desc)+comment+code+command+label & 2 & 3 & 2 & 2 & 3 & 12 \\
HAN(title+desc)+comment+command+label & 3 & 4 & 2 & 1 & 2 & 12 \\
HAN(title+desc)+comment+command & 3 & 3 & 3 & 1 & 2 & 12 \\
HAN(title+desc) & 2 & 4 & 3 & 3 & 1 & 13 \\
HAN(title+desc)+command+label & 3 & 4 & 4 & 1 & 1 & 13 \\
HAN(title+desc)+comment+code+label & 3 & 3 & 2 & 2 & 3 & 13\\
        \bottomrule
        \end{tabular}
        \caption{ScottKnottESD Rank Sum}
        \label{tab:week2}
     \end{subtable}
\end{table}

==> tab/exp3.tex <==
\begin{table}[h]
    \footnotesize
    \label{tab:temps}
    \caption{The result of experiemnt 3.}
    \setlength{\tabcolsep}{1mm}
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{llllllllllllll}
\toprule
 \textbf{Approaches}& \rotatebox{90}{\textbf{TensorFlow}} &  \rotatebox{90}{\textbf{PyTorch}} & \rotatebox{90}{\textbf{Keras}} & \rotatebox{90}{\textbf{Mxnet
}} & \rotatebox{90}{\textbf{Caffe}}\\
\midrule
TF-IDF + KNN & 0.646 & 0.581 & 0.584 & 0.625 & 0.564 &  \\
TF-IDF + MLP & 0.754 & 0.609 & 0.680 & 0.622 & 0.510 &  \\
TF-IDF + RF & 0.601 & 0.513 & 0.568 & 0.500 & 0.500 &  \\
TF-IDF + SVM & 0.661 & 0.500 & 0.541 & 0.500 & 0.500 &  \\
% \textbf{PERCENT} & 13.0\% & 0.2\% & 28.0\% & 0.9\% & 0.9\% & 1.4\% & 7.2\% & 4.4\% & 5.6\% & 8.4\% & 5.4\% & 24.7\%\\
\bottomrule
\end{tabular}
       \caption{AUC Values}
       \label{tab:week1}
    \end{subtable}
    \hfill
    \begin{subtable}[h]{0.5\textwidth}
        \centering
        \begin{tabular}{llllllllllllll}
        \toprule
        \textbf{Approaches}& \rotatebox{90}{\textbf{TensorFlow}} &  \rotatebox{90}{\textbf{PyTorch}} & \rotatebox{90}{\textbf{Keras}} & \rotatebox{90}{\textbf{Mxnet
        }} & \rotatebox{90}{\textbf{Caffe}}&  \rotatebox{90}{\textbf{RankSum}}\\
        \midrule
TF-IDF + KNN &  &  &  &  &  &  \\
TF-IDF + MLP &  &  &  &  &  &  \\
TF-IDF + RF &  &  &  &  &  &  \\
TF-IDF + SVM &  &  &  &  &  &  \\ 
        \bottomrule
        \end{tabular}
        \caption{ScottKnottESD Rank Sum}
        \label{tab:week2}
     \end{subtable}
     
\end{table}



==> tab/false_pos.tex <==
\begin{table}[t!]
\caption{Example of texts extracted from the content of a non-performance bug report for \texttt{TensorFlow}. The \setlength{\fboxsep}{0.5pt}\colorbox{steel!30}{blue} words \texttt{'speed'} and \texttt{'slowed'} contribute the most in identifying as an performance bug report while the \setlength{\fboxsep}{0.5pt}\colorbox{yellow!30}{yellow} words contribute to identify as non-performance bug report.}
\label{tab:false_pos}
\centering
\small
\begin{tabular}{p{8.1cm}}

\toprule
\textbf{Title:} Input Pipeline for \setlength{\fboxsep}{0.5pt}\colorbox{steel!30}{High}-\setlength{\fboxsep}{0.5pt}\colorbox{steel!30}{performance} Model.

\textbf{Comment:} This question is better asked on StackOverflow since it is \setlength{\fboxsep}{0.5pt}\colorbox{yellow!30}{not} a \setlength{\fboxsep}{0.5pt}\colorbox{yellow!30}{bug} or feature request.\\
\bottomrule
\end{tabular}
%}
%\centering
%  \begin{tablenotes}
%     \footnotesize
%      \item The \textcolor{blue!50}{blue}/bold texts are the inputs from the user, where \textcolor{blue!50}{\textbf{\$name}} and \textcolor{blue!50}{\textbf{\$pass}} denote the variable of the username and password given by an user, respectively. The highlighted texts are what will be commented out by the injection attacks.
%     \end{tablenotes}
\end{table}

==> tab/variants-new.tex <==
\begin{table}[t!]
\centering
  \caption{Aliases for different combinations of feature types in \approach. \approach$_A$ is essentially the classic HAN. The \textit{content} feature is handled by the best scheme from RQ1.}
  \label{tb:feature-type}
     \setlength{\tabcolsep}{0.1mm}
  \footnotesize
  \begin{tabular}{llll}
    \toprule
    \textbf{Alias}&\textbf{Feature Types}& \textbf{Alias}&\textbf{Feature Types}\\
    \midrule
    
    \approach$_A$&\textit{content}&\approach$_I$&\textit{content}, \textit{code}, \textit{command}\\
    % \approach$_A$&\textit{comment}\\
    % \approach$_A$&\textit{code}\\
    % \approach$_A$&\textit{command}\\
    % \approach$_A$&\textit{label}\\
    \approach$_B$&\textit{content}, \textit{comment}&\approach$_J$&\textit{content}, \textit{code}, \textit{label}\\
    \approach$_C$&\textit{content}, \textit{code}& \approach$_K$&\textit{content}, \textit{command}, \textit{label}\\
    \approach$_D$&\textit{content}, \textit{command}&\approach$_L$&\textit{content}, \textit{comment}, \textit{command}, \textit{label}\\
    \approach$_E$&\textit{content}, \textit{label}&\approach$_M$&\textit{content}, \textit{comment}, \textit{command}, \textit{code}\\
    \approach$_F$&\textit{content}, \textit{comment}, \textit{code}& \approach$_N$&\textit{content}, \textit{comment}, \textit{code}, \textit{label}\\
    \approach$_G$&\textit{content}, \textit{comment}, \textit{command}& \approach$_O$&\textit{content}, \textit{command}, \textit{code}, \textit{label}\\
    \approach$_H$&\textit{content}, \textit{comment}, \textit{label}& \approach$_P$&\textit{content}, \textit{comment}, \textit{command}, \textit{code}, \textit{label}\\
    
  
  \bottomrule
 \end{tabular}

\end{table}
